On the Design and Security of Collective Remote Attestation Protocols

Collective remote attestation (CRA) is a security service that aims to efficiently identify compromised (often low-powered) devices in a (heterogeneous) network. The last few years have seen an extensive growth in CRA protocol proposals, showing a variety of designs guided by different network topologies, hardware assumptions and other functional requirements. However, they differ in their trust assumptions, adversary models and role descriptions making it difficult to uniformly assess their security guarantees. In this paper we present Catt, a unifying framework for CRA protocols that enables them to be compared systematically, based on a comprehensive study of 40 CRA protocols and their adversary models. Catt characterises the roles that devices can take and based on these we develop a novel set of security properties for CRA protocols. We then classify the security aims of all the studied protocols. We illustrate the applicability of our security properties by encoding them in the tamarin prover and verifying the SIMPLE+ protocol against them.

==> categorisation-a.tex <==
%!TeX root = main.tex
% \section{Categorising CRA Protocols}\label{sec:categories}

%we discuss the categorisation of CRA protocols 
%with respect to: (1) how swarms are organised and clarifying the trust assumption with respect to the verifier, and (2) %several categories that allow us to clearly separate 
%how information from the provers is gathered, which device initiates the protocol, which device is responsible for validating the information from the provers, whether all the provers need to be part of the protocol, and what finer level information about the measurements must be gathered about the provers. 


%The remainder of this section discusses what is meant by each of the metrics in the table in more detail and clarifies whether they are metrics that are extant in the literature or newly identified ones %metrics in this paper 
%in order to provide a fine-grained comparison of the protocols.

%We begin by discussing how swarms are organised and the verifier's trust assumptions in \cref{subsec:topology}, \cref{subsec:dynamicity}, \cref{subsec:centralised} and \cref{subsec:verifier type} respectively. 

%Note that we mentioned in~\cref{sec:intro} Kuang et al introduced the notion of aggregation pattern and topology. We found this terminology confusing and prefer in this paper to refer to the arrangement of devices in a swarm as {\it topology} and use {\it dynamicity} to represent the level of dynamicity of a swarm, as we feel this is more intuitive.

% In this section, we evaluate the identified 40 protocols against 7
% metrics, whose terminology will be later used in the security properties' definitions and examples in \cref{sec:security properties}.  One of the metrics is QoSA, which has already been investigated in the
% literature, but the others are introduced as mertics in this paper for the first time\footnote{More mertrics such as topology  (see~\cref{subsec:topology}), dynamicity (see~\cref{subsec:dynamicity}), and centralisation (see~\cref{subsec:centralised}) as well as a full catergorisation of CRAs (see~\cref{table:categories-OLD}) can be found in Appendix.}. The notation for the values in~\cref{table:categories} are
% explained in the following sub-sections that explain each
% metric. Recall that we have already described some of these metrics: delegated trusted party (see~\cref{subsec:threats to verifier
%   integrity}), validator (see~\cref{subsec:threats to verifier
%   integrity}), attestation target (see~\cref{subsec:threats to prover integrity}), and device availability (see~\cref{subsec:mitigation-detection}). The rest are as
% follows.
% %  (also see columns 6, 11, and 12 in \cref{table:categories}). 















%
%Interactive protocols are good fit in settings where verifiers make
%decisions based on some event, e.g., when an {\em intrusion detection
%system} shows that a prover is suspected of being
%compromised~\cite{leveraging,trust}, or when a monitoring mechanism 
%decides to request attestation on-demand \cite{erasmus(extended)}. 
%However, %in most scenarios, 
%attestation is often used as a standalone
%technique for monitoring untrusted provers and maintenance of a swarm
%so non-interactive protocols can be used to reduce energy cost,
%communication overhead, and run-time. They
%%\sa{and interactive prover (Interactive-P) protocols} 
%can also mitigate computational DoS attacks, as there is no attestation
%request that originates from the verifier (e.g., \seed~\cite{seed}).
%
%Noninteractive-C protocols further 
%decouple the frequency of a verifier’s requests from the frequency of a
%prover’s measurements allowing implementation of a simple collection
%phase 
%%that does not involve any online computation 
%on the provers
%(e.g., \erasmus~\cite{erasmus}). This makes them suitable for highly
%dynamic swarms and for devices working under real-time constraints, 
%% (e.g., safety-critical operations whose proper recognition, control,
%% performance, or tolerance is essential to ensuring safety)
%since the provers will not be distracted from performing their main tasks by
%authenticating new requests and preparing %(aggregated) 
%reports regularly.
%
%
%Non-interactive protocols make both provers and
%verifiers rely on a {\em secure random seed} shared 
%%between every device 
%among all devices
%and stored in their protected memory. % , \sa{which increases the memory cost about 20-byte on an architecture such as \smart~\cite{seed}.} 
%This seed is used to generate a pseudorandom sequence of
%attestation times using a secured {\em Reliable Read-only Clock},
%preventing adversaries from anticipating the next attestation
%%round
%procedure~\cite{seed}.





% so the attacker will not be able
% to infect a device and erase all traces of its previous presence on
% prover before the next attestation round starts. 

%
% An interactive version of \erasmus is
%\erasmusod~\cite{erasmus(extended)} where \erasmus is combined with
%on-demand attestation to benefit from advantages of both
%self-measurement and interactive approaches.

%shela --->The Root Verifier (Vrf): This is the owner of the network that runs the attestation.

% \subsection{Validator}\label{subsec:validator}

% \sr{This is a crucial step in the protocol and the validator should be
% considered in the discussion on trust assumptions. I think this
% section should be moved into Section 3.}

% After a prover generates a measurement there are many options for
% validating whether it matches an expected one (i.e.,
% a healthy status). We classify these as follows (see column 9 in~\cref{table:categories} and \cref{app:validator} for more details).
% \begin{description}[itemsep=0pt,
% leftmargin=0pt]
% \item [Self] protocols, where the measurement is validated by prover
% itself. The prover's attestation result indicates the output of the validation
% (typically Boolean flag indicating whether the prover is
% healthy). The prover therefore needs to know the set of expected
% measurements, and here there are two options: (1) {\it Self verifier} (Self-V)
% protocols, where a verifier sends the set of expected measurements
% to provers, and (2) {\it Self local} (Self-L) protocols where the expected
% measurements are stored locally within the prover itself.
% \item [External] protocols, where the provers send their measurements
% to a third party %that performs the validation.
% to validate. 
% We classify these
% %into subcategories: 
% as follows: (1) {\it Verifier} protocols, where the
% measurements are validated by a centralised verifier, (2) {\it Neighbour}
% protocols, where the measurements are validated by the prover's neighbouring provers, and (3) {\it Jury} protocols, where the measurements are
% validated by a jury of provers.
% \end{description}
% %
% %
% %\mbox{Self} (e.g., \pads~\cite{pads}) and \mbox{neighbour} protocols (e.g.,
% %\pasta~\cite{pasta}) suit settings where provers have sufficient
% %memory to store the expected measurements, and enough computational
% %power to compare their attestation results, thus, leaving less work
% %for a verifier to do. 
% %%\sa{A neighbour prover can be 
% %%physically neighbour (in the same communication range) such as in \usaid~\cite{us-aid} or a logical neighbour such as in \hola~\cite{hola},
% %%where each device is identified by an m-bit number computed by a hash function; and using these identifiers, devices are linked to their predecessors and successors, thus creating a ring.}
% %CRA protocols with no central
% %verifier apply neighbour attestation to
% %distribute the attestation responsibility to all provers (e.g., \hola~\cite{hola}). 
% %\mbox{Self-V} protocols enable a verifier to send the updated expected measurements to provers as needed, but with an additional communication cost since such measurements are included in every attestation request.
% %\mbox{Verifier} protocols are most widely used CRAs for
% %low-end resource
% %constrained devices~\cite{Ambrosin}, since a verifier with additional memory and computation power
% %can be chosen (e.g., \cora~\cite{cora}). \mbox{Jury} protocols are recommended
% %when there is no trusted verifier (e.g., \sadan~\cite{sadan}).
% %
% %
% %The following two metrics: {\it attestation set} and {\it attestation target} are new metrics for CRA protocols.




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


